High density QCD and nucleus-nucleus scattering deeply in the saturation region

In this paper we solve the equations that describe nucleus nucleus scattering, in high density QCD,in the framework of the BFKL Pomeron calculus. We found that (i) the contribution of short distances to the opacity for nucleus-nucleus scattering dies at high energies, (ii) the opacity tends to unity at high energy, and (iii) the main contribution that survives comes from soft (long distance) processes for large values of the impact parameter. The corrections to the opacity $\Omega\Lb Y,b\Rb = 1$ were calculated and it turns out that they have a completely different form, namely($1 - \Omega \to \exp\Lb - Const\,\sqrt{Y}\Rb$) than the opacity that stems from the Balisky-Kovchegov equation, which is($1 - \Omega \to \exp\Lb - Const\,Y^2\Rb$). We reproduce the formula for the nucleus-nucleus cross section that is commonly used in the description of nucleus-nucleus scattering, and there is no reason why it should be correct in the Glauber-Gribov approach

==> eqAA-ref_upd.tex <==
\begin{thebibliography}{99}
\bibitem{GLR}
L. V. Gribov, E. M. Levin and M. G. Ryskin, 
Phys. Rep. {\bf 100} (1983) 1. 
\bibitem{MUQI}
A. H. Mueller and J. Qiu,
Nucl. Phys. {\bf B268} (1986) 427.
\bibitem{MV}
L. McLerran and R. Venugopalan, 
Phys. Rev. {\bf D49} (1994) 2233, 3352; {\bf D50} (1994) 2225; 
{\bf D53} (1996) 458;\\ {\bf D59} (1999) 09400. 
\bibitem{MUCD}
 A.~H.~Mueller,
  %``Soft Gluons In The Infinite Momentum Wave Function And The Bfkl Pomeron,''
  Nucl.\ Phys.\  B {\bf 415}, 373 (1994); 
 %``Unitarity and the BFKL pomeron,''
  Nucl.\ Phys.\  B {\bf 437} (1995) 107
  [arXiv:hep-ph/9408245].
  %%CITATION = NUPHA,B415,373;%%
  %%CITATION = NUPHA,B437,107;%
\bibitem{B}
I.~Balitsky,
[arXiv:hep-ph/9509348];\,\,
%%CITATION = HEP-PH 9509348;%%
{\it Phys.\ Rev.} {\bf D60}, 014020 (1999)
[arXiv:hep-ph/9812311]\,\,\,\,
%%CITATION = HEP-PH 9812311;%%
\bibitem{K}
Y.~V.~Kovchegov,
{\it Phys.\ Rev.}  {\bf D60}, 034008  (1999),
[arXiv:hep-ph/9901281].
%%CITATION = HEP-PH 9901281;%%
\bibitem{JIMWLK}
~J.~Jalilian-Marian, A.~Kovner, A.~Leonidov and H.~Weigert,
{\it  Phys.\ Rev.}\,  {\bf D59}, 014014 (1999),
[arXiv:hep-ph/9706377];\,\,  {\it Nucl.\ Phys.}\,{\bf B504}, 415
(1997),
[arXiv:hep-ph/9701284]; \,\,\,
J.~Jalilian-Marian, A.~Kovner and H.~Weigert,
  {\it Phys.\ Rev.}  {\bf D59}, 014015 (1999),
  [arXiv:hep-ph/9709432];\,\,\,
  %%CITATION = HEP-PH 9709432;%%
 A.~Kovner, J.~G.~Milhano and H.~Weigert,
 {\it  Phys.\ Rev.}  {\bf D62}, 114005 (2000),
  [arXiv:hep-ph/0004014]\,; \,\,\,
  %%CITATION = HEP-PH 0004014;%%
E.~Iancu, A.~Leonidov and L.~D.~McLerran,
{\it  Phys.\ Lett.}\,  {\bf B510}, 133 (2001);
[arXiv:hep-ph/0102009];\,\, {\it  Nucl.\ Phys.}\,  {\bf A692}, 583
(2001),
[arXiv:hep-ph/0011241];\,\,\,
E.~Ferreiro, E.~Iancu, A.~Leonidov and L.~McLerran,
 {\it  Nucl.\ Phys.}\  {\bf A703}, 489 (2002),
  [arXiv:hep-ph/0109115];\,\,\,
  %%CITATION = HEP-PH 0109115;%%
H.~Weigert,
{\it  Nucl.\ Phys.}  {\bf A703}, 823 (2002),
[arXiv:hep-ph/0004044].


\bibitem{BRA}
 M.~A.~Braun,
 Phys.Lett. B 483 (2000) 115, [arXiv:hep-ph/0003004]; \,
  %``Conformal invariant pomeron interaction in the perturbative QCD with  large
  %N(c),''
%'Nucleus-nucleus interaction in pertutbative QCD"
Eur.Phys.J C { \bf 33} (2004) 113  [arXiv:hep-ph/0309293]
;\,
  Phys.\ Lett.\  B {\bf 632} (2006) 297,
  [Eur.\ Phys.\ J.\  C {\bf 48} (2006) 511],
  [arXiv:hep-ph/0512057].
. 
% 'Nucleus-nucleus interaction in pertutbative QCD"

  %%CITATION = HEP-PH/0504002;%%
\bibitem{KOLU}
 T.~Altinoluk, A.~Kovner, M.~Lublinsky and J.~Peressutti,
  %``QCD Reggeon Field Theory for every day: Pomeron loops included,''
  JHEP {\bf 0903} (2009) 109
  [arXiv:0901.2559 [hep-ph]];\,\,\, A.~Kovner and M.~Lublinsky,
  %%CITATION = JHEPA,0903,109;%%
  %``From target to projectile and back again: selfduality of high energy
  %evolution,''
  Phys.\ Rev.\ Lett.\  {\bf 94} (2005) 181603
  [arXiv:hep-ph/0502119];\,\,
\,
  %``In pursuit of pomeron loops: The JIMWLK equation and the Wess-Zumino
  %term,''
  Phys.\ Rev.\  D {\bf 71} (2005) 085004
  [arXiv:hep-ph/0501198].
  %%CITATION = PHRVA,D71,085004;%%
  %%CITATION = PRLTA,94,181603;%
\bibitem{LELU}
 E.~Levin and M.~Lublinsky,
  %``Towards a symmetric approach to high energy evolution: Generating
  %functional with Pomeron loops,''
  Nucl.\ Phys.\  A {\bf 763} (2005) 172
  [arXiv:hep-ph/0501173].
  %%CITATION = NUPHA,A763,172;%%
\bibitem{BIIT}
 J.~P.~Blaizot, E.~Iancu, K.~Itakura and D.~N.~Triantafyllopoulos,
  %``Duality and Pomeron effective theory for QCD at high energy and large
  %N(c),''
  Phys.\ Lett.\  B {\bf 615} (2005) 221
  [arXiv:hep-ph/0502221].
  %%CITATION = PHLTA,B615,221;%%
\bibitem{HIMST}
 Y.~Hatta, E.~Iancu, L.~McLerran, A.~Stasto and D.~N.~Triantafyllopoulos,
  %``Effective Hamiltonian for QCD evolution at high energy,''
  Nucl.\ Phys.\  A {\bf 764} (2006) 423
  [arXiv:hep-ph/0504182].
  %%CITATION = NUPHA,A764,423;%%
\bibitem{MMSW}
 C.~Marquet, A.~H.~Mueller, A.~I.~Shoshi and S.~M.~H.~Wong,
  %``On the projectile-target duality of the color glass condensate in the
  %dipole picture,''
  Nucl.\ Phys.\  A {\bf 762} (2005) 252
  [arXiv:hep-ph/0505229].
  %%CITATION = NUPHA,A762,252;%%
\bibitem{LMP}
  E.~Levin, J.~Miller and A.~Prygarin,
  %``Summing Pomeron loops in the dipole approach,''
  Nucl.\ Phys.\  A {\bf 806} (2008) 245
  [arXiv:0706.2944 [hep-ph]].
  %%CITATION = NUPHA,A806,245;%%
\bibitem{BOMO}
S.~Bondarenko and L.~Motyka,
  %``Solving effective field theory of interacting QCD pomerons in the
  %semi-classical approximation,''
  Phys.\ Rev.\  D {\bf 75} (2007) 114015
  [arXiv:hep-ph/0605185].
  %%CITATION = PHRVA,D75,114015;%%
\bibitem{BOBR}
 S.~Bondarenko and M.~A.~Braun,
  %``Boundary conditions in the QCD nucleus-nucleus scattering problem,''
  Nucl.\ Phys.\  A {\bf 799} (2008) 151
  [arXiv:0708.3629 [hep-ph]].
  %%CITATION = NUPHA,A799,151;%%
\bibitem{BFKL}
 E. A. Kuraev, L. N. Lipatov, and F. S. Fadin, {\it  Sov. Phys.
JETP}
                {\bf 45}, 199 (1977); \,\,\,
Ya. Ya. Balitsky and L. N. Lipatov,
               {\it   Sov. J. Nucl. Phys.}\, {\bf 28}, 22 (1978).

\bibitem{LI}
L. N. Lipatov,
Phys. Rep. {\bf 286} (1997) 131; Sov. Phys. JETP {\bf 63} (1986) 904 
and references therein. 
\bibitem{KLP}
 M.~Kozlov, E.~Levin and A.~Prygarin,
  %``The BFKL Pomeron Calculus in the dipole approach,''
  Nucl.\ Phys.\  A {\bf 792}, 122 (2007)
  [arXiv:0704.2124 [hep-ph]];\,\,{\it ``The BFKL pomeron calculus: Probabilistic interpretation and high energy
  amplitude,''}
  arXiv:hep-ph/0606260.
  %%CITATION = HEP-PH/0606260;%%

  %%CITATION = NUPHA,A792,122;%%
\bibitem{SCHW}
 A.~Schwimmer,
  %``Inelastic Rescattering And High-Energy Reactions On Nuclei,''
  Nucl.\ Phys.\  B {\bf 94} (1975) 445.
  %%CITATION = NUPHA,B94,445;%%

\bibitem{GKLM}
E.~Gotsman, A.~Kormilitzin, E.~Levin and U.~Maor,
  %``QCD motivated approach to soft interactions at high energies:
  %nucleus-nucleus and hadron-nucleus collisions,''
  Nucl.\ Phys.\  A {\bf 842} (2010) 82
  [arXiv:0912.4689 [hep-ph]].
  %%CITATION = NUPHA,A842,82;%%

\bibitem{GLAUB}
R.J.Glauber, in {\it  ``Lectures in Theoretical Physics"}, edited by by W. E. Britten et al. (Interscience, New York) {\bf 1}, (1959) 315.
\bibitem{KOWI}
 A.~Kovner and U.~A.~Wiedemann,
%``No Froissart bound from gluon saturation,''
  Phys.\ Lett.\  B {\bf 551} (2003) 311
  [arXiv:hep-ph/0207335];\,\,
  %%CITATION = PHLTA,B551,311;%%
  %``Perturbative saturation and the soft pomeron,''
  Phys.\ Rev.\  D {\bf 66} (2002) 034031
  [arXiv:hep-ph/0204277];\,\,
  %%CITATION = PHRVA,D66,034031;%%
  %``Nonlinear QCD evolution: Saturation without unitarization,''
  Phys.\ Rev.\  D {\bf 66} (2002) 051502
  [arXiv:hep-ph/0112140].
  %%CITATION = PHRVA,D66,051502;%%
\bibitem{MUSH}
 A.~H.~Mueller and A.~I.~Shoshi,
  %``Small-x physics beyond the Kovchegov equation,''
  Nucl.\ Phys.\  B {\bf 692} (2004) 175
  [arXiv:hep-ph/0402193].
  %%CITATION = NUPHA,B692,175;%%

\bibitem{MUTR}
A.~H.~Mueller and D.~N.~Triantafyllopoulos,
{\it Nucl.\ Phys.}\,  {\bf B640} (2002) 331
[arXiv:hep-ph/0205167];\,\,\,\,D.~N.~Triantafyllopoulos,
{\it Nucl.\ Phys.}\, {\bf B648} (2003) 293
[arXiv:hep-ph/0209121].
%%CITATION = HEP-PH 0209121;%%
%%CITATION = HEP-PH 0205167;%%

\bibitem{MP}
S.~Munier and R.~Peschanski,
{\it Phys.\ Rev.}\,  {\bf D70} (2004) 077503;
 {\bf D69} (2004) 034008
[arXiv:hep-ph/0310357];\,\,
{\it Phys.\ Rev.\ Lett.}\,  {\bf 91} (2003) 232001
[arXiv:hep-ph/0309177].
\bibitem{LTSOL}
  E.~Levin and K.~Tuchin,
  %``Solution to the evolution equation for high parton density QCD,''
  Nucl.\ Phys.\  B {\bf 573} (2000) 833
  [arXiv:hep-ph/9908317].
  %%CITATION = NUPHA,B573,833;%%
\bibitem{ELRE}
 E.~Levin,
  %``Renormalons at low x,''
  Nucl.\ Phys.\  B {\bf 453} (1995) 303
  [arXiv:hep-ph/9412345].
  %%CITATION = NUPHA,B453,303;%%
\bibitem{MBK}
E.~Gotsman, E.~Levin, U.~Maor and E.~Naftali,
  %``A modified Balitsky-Kovchegov equation,''
  Nucl.\ Phys.\  A {\bf 750} (2005) 391
  [arXiv:hep-ph/0411242].
  %%CITATION = NUPHA,A750,391;%%
\bibitem{DG}
 V.~A.~Khoze, A.~D.~Martin, M.~G.~Ryskin and W.~J.~Stirling,
  %``The spread of the gluon k(t)-distribution and the determination of the
  %saturation scale at hadron colliders in resummed NLL BFKL,''
  Phys.\ Rev.\  D {\bf 70} (2004) 074013
  [arXiv:hep-ph/0406135].
  %%CITATION = PHRVA,D70,074013;%%
\bibitem{LTA}
 E.~Levin and K.~Tuchin,
  %``Nonlinear evolution and saturation for heavy nuclei in DIS,''
  Nucl.\ Phys.\  A {\bf 693} (2001) 787
  [arXiv:hep-ph/0101275].
  %%CITATION = NUPHA,A693,787;%%
\bibitem{IAMU}
E. Iancu and A. H. Mueller,
Nucl. Phys. {\bf A730} (2004) 460 [arXiv:hep-ph/0308315];            
494 [arXiv:hep-ph/0309276].

\bibitem{RY}
I. Gradstein and I. Ryzhik, 
{\it "Tables of Series, Products, and Integrals"}, Verlag MIR, Moskau,1981.

\bibitem{QSA}
A.~H.~Mueller,
  %``Nuclear A-dependence near the saturation boundary,''
  Nucl.\ Phys.\  A {\bf 724} (2003) 223
  [arXiv:hep-ph/0301109];%``Parton saturation at small x and in large nuclei,''
  Nucl.\ Phys.\  B {\bf 558} (1999) 285
  [arXiv:hep-ph/9904404];
  %%CITATION = NUPHA,B558,285;%%\,\,\,
D.~Kharzeev, E.~Levin and L.~McLerran,
  %``Parton saturation and N(part) scaling of semi-hard processes in QCD,''
  Phys.\ Lett.\  B {\bf 561} (2003) 93
  [arXiv:hep-ph/0210332];\,\,\, E.~M.~Levin and M.~G.~Ryskin,
  %``The Hadron - Nucleus Interaction In QCD At High-Energy,''
  Nucl.\ Phys.\  B {\bf 304} (1988) 805; 
  %``Deep Inelastic Scattering On Nuclei At Small X. (In Russian),''
  Sov. J. Nucl. Phys. 41 (1985) 472.
  %%CITATION = YAFIA,41,472;%%
  %%CITATION = NUPHA,B304,805;%%
  %%CITATION = PHLTA,B561,93;%%
  %%CITATION = NUPHA,A724,223;%%


\bibitem{FROI}
M.~Froissart,
{\it Phys.\, Rev.} \,  {\bf 123} (1961) 1053; \\
~A. ~Martin, {``Scattering Theory: Unitarity, Analitysity and Crossing."}
Lecture Notes in Physics, Springer-Verlag,  Berlin-Heidelberg-New-York,
1969.







\bibitem{GRIBA}
R.J. Glauber, In: Lectures in Theor. Phys., v. 1, ed. W.E. Brittin and L.G. Duham. NY: Intersciences, 1959;\,\,\,
  Gribov,~V.~N.,
Sov.\ Phys.\ JETP\,{\bf 29} 483,
  [Zh.\ Eksp.\ Teor.\ Fiz.\,  {\bf 56} 892 (1969)];
Sov.\ Phys.\ JETP\,{\bf 30} 709
  [Zh.\ Eksp.\ Teor.\ Fiz.\ \, { \bf  57} (1969) 1306].
  %%CITATION = ZETFA,57,1306;%%

\bibitem{GG}
 A.~Kaidalov,
  %``Nucleus nucleus interaction dynamics and the Glauber-Gribov approach,''
  Nucl.\ Phys.\  A {\bf 525} (1991) 39;\,\,
  %%CITATION = NUPHA,A525,39;%%
 K.~G.~Boreskov and A.~B.~Kaidalov,
  %``Nucleus-Nucleus Scattering In The Glauber Approach,''
  Sov.\ J.\ Nucl.\ Phys.\  {\bf 48} (1988) 367
  [Yad.\ Fiz.\  {\bf 48} (1988) 575];\,
  %``NUCLEUS-NUCLEUS INTERACTIONS IN THE GLAUBER APPROACH,''
  Acta Phys.\ Polon.\  B {\bf 20} (1989) 397 and references therein.
  %%CITATION = APPOA,B20,397;%%
  %%CITATION = YAFIA,48,575;%%


\end{thebibliography}


